Colorful Image Colorization

Given a grayscale photograph as input, this paper attacks the problem of hallucinating a plausible color version of the photograph. This problem is clearly underconstrained, so previous approaches have either relied on significant user interaction or resulted in desaturated colorizations. We propose a fully automatic approach that produces vibrant and realistic colorizations. We embrace the underlying uncertainty of the problem by posing it as a classification task and use class-rebalancing at training time to increase the diversity of colors in the result. The system is implemented as a feed-forward pass in a CNN at test time and is trained on over a million color images. We evaluate our algorithm using a "colorization Turing test," asking human participants to choose between a generated and ground truth color image. Our method successfully fools humans on 32% of the trials, significantly higher than previous methods. Moreover, we show that colorization can be a powerful pretext task for self-supervised feature learning, acting as a cross-channel encoder. This approach results in state-of-the-art performance on several feature learning benchmarks.

==> commands.tex <==
\definecolor{MyDarkBlue}{rgb}{0,0.08,0.5}
\definecolor{MyLightBlue}{rgb}{0,0.08,0.8}
\definecolor{MyDarkGreen}{rgb}{0.02,0.50,0.02}
\definecolor{MyDarkRed}{rgb}{0.7,0.02,0.02}
\definecolor{MyDarkOrange}{rgb}{0.40,0.2,0.02}
\definecolor{MyDarkMagenta}{rgb}{0.337,0,0.827}
\newcommand{\PhillipComment}[1]{\textcolor{MyLightBlue}{Phillip:  ``#1"}}
\newcommand{\RichardComment}[1]{\textcolor{MyDarkMagenta}{Richard:  ``#1"}}



==> intro.tex <==

Consider the grayscale photographs in the top row of Figure~\ref{fig:teaser}.  At first glance, hallucinating what they would look like in color seems a daunting task, since so much of the information (two out of the three dimensions) has been lost! But looking more closely, one notices that in many cases, the semantics of the scene, together with the surface texture, provides ample cues for many regions in each image: the grass is typically green, the sky is typically blue, and the strawberry that has been photographed with a such inviting close-up, is most likely bright red. Of course, this kind of semantic prior doesn't work for everything, e.g., the finish line sign in the second image doesn't have to be red. However, for this paper, our goal is not to necessarily recover the actual ground truth color, but rather to produce a {\em plausible} colorization that could potentially fool a human observer. Therefore, our task becomes a much more achievable one: to model enough of the statistical dependencies between the semantics and the textures of grayscale images and their color versions to produce visually compelling results.

%take a grayscale image and produce at least one high probability sample from the conditional distribution $P(ab | l)$. 

%This is related to the problem of generative image modeling, but easier since we 

Given a luminance map, our system predicts its $a$ and $b$ color channels in $Lab$ colorspace. To solve this problem, we leverage large-scale data. Predicting color has the nice property that training data is very cheap: any color photo can be used as a training example simply by taking the image's $L$ channel as input its $ab$ channels as target output. Others have noted the availability of training data and trained Convolutional neural networks (CNNs) to predict color on large datasets \cite{cheng2015deep,dahl2016tinyclouds}.

However, the results from these and other past attempts tend to look bland and desaturated (see Figures \ref{fig:imagenet_comparison} and \ref{fig:learch_comparison}). One explanation is that \cite{cheng2015deep} and \cite{dahl2016tinyclouds} use loss functions that encourage conservative results. These losses are inherited from standard regression problems, where the goal is to minimize Euclidean error between an estimate and the ground truth.

We instead design a loss that embraces the inherent ambiguity in color prediction. We formulate the colorization problem as multinomial classification, predicting a distribution of possible colors at each pixel. Further, we re-weight the loss to emphasize rare colors. This encourages our model to exploit the full diversity of the large-scale data on which it is trained. The end result is colorizations that are more vibrant and perceptually compelling than those of previous approaches.

%and aims to create more perceptually compelling and \emph{colorful} colorizations. Paired with large scale data, our method can learn a large diversity of .

%To synthesize plausible colors, it is important to recognize that color, in many cases, is more ambiguous than popular 


%Colorization is the task of predicting the color of an image given the color in grayscale. To successfully color a black and white image, one must combine low-level cues with high-level semantic cues, along with prior knowledge regarding the distribution of colors of objects. Convolutional neural networks (CNNs) have considerably advanced the state-of-the-art in many tasks in computer vision. 

%However, previous attempts at applying CNNs to the task of colorization~\cite{cheng2015deep}~\cite{dahl2016tinyclouds} have resulted in bland and desaturated outputs. More colorful results can be achieved using methods that required strong user interaction, either in selecting reference images[][][][], providing metadata for the image, or providing colorized brush strokes~\cite{levin2004colorization}. In this paper, we aim for a completely automatic method, that nonetheless creates realistic and \emph{colorful} colorizations.

\begin{figure}[t]
 \centering
 \includegraphics[width=1.0\hsize]{imgs/teaser2.pdf}
  \caption{Example input and output from our algorithm. Best viewed in color\footnotemark.}
 \label{fig:teaser}
\end{figure}
%\footnotetext{\PhillipComment{(figure out how to rotate this)} Answer: all are fake.}
\footnotetext{obviously}

%How do we contrast with other methods?

%What are our contributions?
%1. Colorfulness
%    -- classification loss
%    -- class-rebalancing
%2. High capacity net, big data
%3. Evaluation


%We treat the colorization problem as a conditional generation problem. Given a luminance map, our system predicts its $a$ and $b$ color channels in $lab$ colorspace. We embrace the inherit ambiguity of the problem by treating the problem as a classification problem, predicting a distribution of possible colors at each pixel. Although the world around us may appear quite lively, the vast majority of pixels in natural images actually reside in a desaturated region of color space (see Figure \ref{XX}). To encourage the CNN to produce vibrant and colorful outputs, we perform class-rebalancing at training time. Our CNN uses convolution and downsampling layers, followed by upsampling and convolution, in the style of a convolutional autoencoder. We use dilation~\cite{yu2015multi} in the middle layers to maintain additional spatial resolution in the network bottleneck, along with BatchNorm layers ~\cite{ioffe2015batch} to better condition network optimization. We perform inference by interpolating between the mean of the predicted distribution, which is more spatially consistent but less vibrant, and mode of the learned distribution, which is vibrant but sometimes incorrect.

Evaluating the quality of synthesized images is notoriously difficult. Since our ultimate goal is to make results that are compelling to a human observer, we introduce a novel way of evaluating colorization results, directly testing their perceptual realism. We setup a ``colorization Turing test" in which we show participants real and synthesized colors for a photo, and ask them which is which. In this paradigm we are able to fool participants $21\%$ of the time, significantly higher than alternative algorithms; the test demonstrates that in many cases, our algorithm is producing nearly photorealistic results (see Figure \ref{fig:teaser} for selected successful results from our algorithm).

%In addition to our model and algorithm, an important contribution of our paper is a novel framework for evaluating colorization results. 

Our contributions in this paper are to 1) set a new high watermark on the task of automatic image colorization, by learning from a million photos, 2) design an objective function appropriate for the colorization problem that handles the inherent uncertainty in the problem and captures a wide diversity of colors, and 3) introduce a novel framework for testing image synthesis algorithms.

%To evaluate our algorithm, we use three quantitative metrics with increasing abstraction towards perceptual realism. (1) We account for percentage of predicted pixels below a threshold in euclidean distance in ab space. This metric is highly limited, and will mostly contain desaturated background pixels. To correct for this, we also evaluate on a color-class-balanced version of this metric. (2) Per-pixel accuracy will never account for whether a generated colorization is perceptually realistic. We take a step towards evaluating perceptual realism by using the VGG classification network~\cite{simonyan2014very} as a perception model. We evaluate the classification accuracy of the VGG classification network before and after colorization. This metric reveals which classes are successfully recolored in a way interpretable to VGG. (3) We further evaluate the realism of our prediction by proposing a visual Turing test. We flash images of a ground truth colorization, along with the output of our system on Amazon Mechanical Turk, and ask the user to choose the synthesized image. We find that we fool the user on 17\% of instances. 

%You can attempt a version of this test right now for yourself. Consider Figure \ref{fig:fig1}. Real photographs are mixed with example outputs of our algorithm. Can you guess which images are generated and which are real?
%along with the classes that VGG has learned to classify primarily based on color

% We treat the problem using a classification framework to account for the inherent ambiguity of the task.

% The input to our system is a grayscale image, the luminance channel of an LAB image. The desired output of the system are the a and b channels of the color space. Convolutional networks for pixel-wise prediction have been well-explored, with architectures such as FCNs [ ], HEDs [ ], and ... making advancements in the tasks of semantic segmentation [ ], segmentation [ ], and surface normal estimation. Our network uses the VGG network in a convolutional autoencoder style, allowing the network to build up sophistication in the front half by increasing its effective dilation. In the second half of the network, the effective dilation is decreased to allow the network to learn spatial consistency. We approach the problem by using a classification approach, which allows the network to fully learn the \textit{distribution} of possible colorings for a given pixel. We then perform our final inference by adjusting the temperature of the softmax and taking the mean of the distribution. A final optional post-processing step is used for slightly more pleasing visual results.

% \begin{itemize}
% \item Percentage of pixels within a threshold
% \item VGG as a perception model
% \item Turk task asking users to discriminate between a generated image and real image
% \end{itemize}

% We test our system on out-of-domain examples and qualitatively show that the method degrades gracefully.

% Consider Figure \ref{fig:fig1}. Is the fruit an orange or a lemon? Is the butterfly orange or blue? Is the woman's scarf pink or green? These examples demonstrate the inherent ambiguity in the colorization problem. To color a black and white image, one must combine low-level cues with high-level semantic cues, along with prior knowledge regarding the distribution of colors of objects. We approach this problem by designing a system which outputs \textit{multiple} modes or possible colorings given a single grayscale image, as shown in Figure \ref{fig:overview}, and by leveraging big data [ ] to learn the distribution of colors of objects. The input of the system is a grayscale image, the luminance channel of an LAB image. We use a convolutional network inspired by the front-end of the VGG-16 network [ ], with pooling layers removed, evaluated densely over \textit{every} pixel in the input image in a fully-convolutional manner, to output a distribution of colors per pixel. The network is trained to classify the color of the center pixel in a large receptive field as a distribution over quantized ab space. A classification approach was taken over a regression approach, since regression does not express the possible colorings of a pixel, but only provides a single point estimate in color space.
